Balanced Depth Completion between Dense Depth Inference and Sparse Range Measurements via KISS-GP

Estimating a dense and accurate depth map is the key requirement for autonomous driving and robotics. Recent advances in deep learning have allowed depth estimation in full resolution from a single image. Despite this impressive result, many deep-learning-based monocular depth estimation (MDE) algorithms have failed to keep their accuracy yielding a meter-level estimation error. In many robotics applications, accurate but sparse measurements are readily available from Light Detection and Ranging (LiDAR). Although they are highly accurate, the sparsity limits full resolution depth map reconstruction. Targeting the problem of dense and accurate depth map recovery, this paper introduces the fusion of these two modalities as a depth completion (DC) problem by dividing the role of depth inference and depth regression. Utilizing the state-of-the-art MDE and our Gaussian process (GP) based depth-regression method, we propose a general solution that can flexibly work with various MDE modules by enhancing its depth with sparse range measurements. To overcome the major limitation of GP, we adopt Kernel Interpolation for Scalable Structured (KISS)-GP and mitigate the computational complexity from O(N^3) to O(N). Our experiments demonstrate that the accuracy and robustness of our method outperform state-of-the-art unsupervised methods for sparse and biased measurements.

==> fig_kitti_sampling.tex <==
% Figure
\begin{figure}[!t]
	\def\width{0.8\columnwidth}%
	\centering
	\subfigure[RGB image]{
		\includegraphics[width=\width]{figs/sampling_rgb.pdf}
		\label{fig:rgb}
	}\\
	\subfigure[Corresponding LiDAR scan (Full FOV)]{
		\includegraphics[width=\width]{figs/sampling_full.pdf}
		\label{fig:full}
	}
	\subfigure[Uniformly sampled scan]{
		\includegraphics[width=\width]{figs/sampling_uniform.pdf}
		\label{fig:uniform}
	}
	\subfigure[Horizontally sampled scan]{
		\includegraphics[width=\width]{figs/sampling_horizontal.pdf}
		\label{fig:horizontal}
	}
	\subfigure[Vertically sampled scan]{
		\includegraphics[width=\width]{figs/sampling_vertical.pdf}
		\label{fig:vertical}
	}
	\caption{Three different sampling methods for the evaluation of spasity and irregularly spaced measurements. \subref{fig:rgb} and \subref{fig:full} The origianl RGB image and LiDAR raw data from KITTI depth completion dataset. \subref{fig:uniform} The uniform sampling is to evaluate the depth interpolation of sparse lidar measurements. \subref{fig:horizontal} and \subref{fig:vertical} The full LiDAR data is subsampled into seven levels of biased measurements. The performance of depth extrapolation can be evaluated with these data. }
	\label{fig:sampling_methods_KITTI}
\end{figure}
% Figure


==> tab_kitti_metric_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\scriptsize
\centering
  \begin{tabular}{c|c|c|c|c|c|c|c|c} \hline
  Point density& \multicolumn{4}{c|}{Ours} & \multicolumn{4}{c}{Ma et al. \cite{Ma2018}} \\ \cline{2-9}
  \# scan line & RMSE [mm] & MAE [mm] & iRMSE [1/km] & iMAE [1/km] &
                 RMSE [mm] & MAE [mm] & iRMSE [1/km] & iMAE [1/km] \\ \hline \hline
  \begin{tabular}[c]{@{}c@{}}1/4x\\ (16)\end{tabular} &
    \textbf{2614.04} &
    \textbf{1141.02} &
    \textbf{14.89} &
    \textbf{5.68} &
    20584.63 &
    13550.55 &
    54.97 &
    43.45 \\ \hline
  \begin{tabular}[c]{@{}c@{}}1/2x\\ (32)\end{tabular} &
    \textbf{1696.34} &
    \textbf{705.02} &
    \textbf{18.17} &
    \textbf{4.36} &
    5741.87 &
    3132.26 &
    45.32 &
    30.65 \\ \hline
  \begin{tabular}[c]{@{}c@{}}full\\ (64)\end{tabular} &
    1593.37 &
    547.00 &
    27.98 &
    2.36 &
    \textbf{1343.33} &
    \textbf{358.66} &
    \textbf{4.28} &
    \textbf{1.64} \\ \hline
  \end{tabular}%
  \caption{Overall results with horizontally sampled data in the KITTI depth completion dataset. The horizontally sampled data is defined as the number of laser scans facing front, as described in \figref{fig:sampling_methods_KITTI}. \hl{unbold multirow}}
  \label{tab:kitti_metric}
\end{table*}

